Reducts of structures and maximal-closed permutation groups

Answering a question of Junker and Ziegler, we construct a countable first order structure which is not omega-categorical, but does not have any proper non-trivial reducts, in either of two senses (model-theoretic, and group-theoretic). We also construct a strongly minimal set which is not omega-categorical but has no proper non-trivial reducts in the model-theoretic sense.

==> macros.tex <==

\def\at{\mathop{\rm at}\nolimits}
\def\gcd{\mathop{\rm g.c.d.}\nolimits}
\def\tp{\mathop{\rm tp}\nolimits}
\def\mod{\mathop{\rm mod}\nolimits}
\def\deg{\mathop{\rm deg}\nolimits}
\def\vert{\mathop{\rm vert}\nolimits}
\font\msbmten msbm10
\def \Bbb#1{\hbox{\msbmten #1}}
\def\Uu{\Bbb U}
\def\Qq {\Bbb Q}  \def\Nn{\Bbb N} \def\Rr {\Bbb R} \def\Cc
{\Bbb C}
\def\Ff{\Bbb F} 
\def\Sup{\mathop{\rm Sup}\nolimits}
\def\supp{\mathop{\rm supp}\nolimits}
\def\AG{\mathop{\rm AG}\nolimits}
\def\AGL{\mathop{\rm AGL}\nolimits}
\def\PG{\mathop{\rm PG}\nolimits}
\def\PGL{\mathop{\rm PGL}\nolimits}

\def\Min{\mathop{\rm Min}\nolimits}
\def\char{\mathop{\rm char}\nolimits}
\def\rings{\mathop{\rm rings}\nolimits}
\def\div{\mathop{\rm div}\nolimits}
\def\Aut{\mathop{\rm Aut}\nolimits}
\def\an{\mathop{\rm an}\nolimits}
\def\mod{\mathop{\rm mod}\nolimits}
\def\Max{\mathop{\rm Max}\nolimits}
\def\Sym{\mathop{\rm Sym}\nolimits}
\def\Wr{\mathop{\rm Wr}\nolimits}
\def\Th{\mathop{\rm Th}\nolimits}
\def\acl{\mathop{\rm acl}\nolimits}
\def\SENT{\mathop{\rm SENT}\nolimits}
\def\dom{\mathop{\rm dom}\nolimits}
\def\ran{\mathop{\rm ran}\nolimits}
\def\unc{\underline{c}}
\def\unF{\underline{F}}
\def\unf{\underline{f}}
\def\unR{\underline{R}}
\def\unS{\underline{S}}
\def\und{\underline{d}}
\def\unP{\underline{P}}
\def\unE{\underline{E}}
\def\calM{{\cal M}}
\def\calA{{\cal A}}
\def\calB{{\cal B}}
\def\calN{{\cal N}}
\def\calR{{\cal R}}
\def\calP{{\cal P}}
\def\calF{{\cal F}}
\def\calZ{{\cal Z}}
\def\la{\langle}
\def\ra{\rangle}
